Multimodal Network Alignment

A multimodal network encodes relationships between the same set of nodes in multiple settings, and network alignment is a powerful tool for transferring information and insight between a pair of networks. We propose a method for multimodal network alignment that computes a matrix which indicates the alignment, but produces the result as a low-rank factorization directly. We then propose new methods to compute approximate maximum weight matchings of low-rank matrices to produce an alignment. We evaluate our approach by applying it on synthetic networks and use it to de-anonymize a multimodal transportation network.

==> 75-genomic.tex <==

\subsection{Protein Protein Interaction Networks from supergenomic network}
In this set of experiments, we have data coming from Biological databases encoding relationships between proteins. We have 7 modes of relationship between the proteins. Namely, these are neighborhood, fusion, cooccurence, coexpression, experimental, database, and text mining. Since each of these modes correspond to a network, we can assemble a multimodal network for each species. We tried running our approach with the matrix $\mL$ as described in~\ref{matrixL}, but since these networks are Biological networks that do not necessairly align perfectly we needed a better low-rank similarity measure. We used COGs [XXX describe more] data... 
[XXX very sloppy here... just writing down the idea]
take rank 1 appx, 10 appx, 25 appx. use these to do multimodal alignment
recreate the COG with the 1appx, 10appx, 25appx... Remove all vals $<10^-4$ (to make it sparse/faster), run netalignmr on these

For each, record: (1) time, (2) nb of conserved edges, (3) number of edges that were aligned and turned out to be true COG edges

I report all the values in the following table... Might need to have a plot. But this also supports multimodality..

\begin{table}[h]
\centering
\begin{tabular}{rlll}
\toprule
\textbf{mode}									& k=1 & k=10& k=25\\ \toprule
smashed(conserved edges)			& 222    &     1332  &       2076\\
smashed(time)								&17.738    &   137.19  &     144.11\\
smashed(COGs predicted)				&           153      &    465      &    743\\
multi(conserved edges)					& 2674     &   18386  &      27354\\
multi(time)										& 0.33325    &   17.377 &      93.903\\
multi(COGs predicted)                  	& 168    &      979      &   1445\\ \bottomrule
\end{tabular}
\label{tab:3}
\caption{Mouse Chimpanzee, total edges = 129862}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{rlll}
\toprule
\textbf{mode}									& k=1 & k=10& k=25\\ \toprule
smashed(conserved edges)			&  412     &    1002      &   2234\\
smashed(time)								& 47.661   &    108.78   &    217.04\\
smashed(COGs predicted)				& 197      &    451       &   726\\
multi(conserved edges)					&4248      &  22554     &   25658\\
multi(time)										& 0.35025  &     15.749  &     22.883\\
multi(COGs predicted)                  	& 243      &   1221   &      1452\\ \bottomrule
\end{tabular}
\label{tab:4}
\caption{Human Chimpanzee.98038}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{rlll}
\toprule
\textbf{mode}									& k=1 & k=10& k=25\\ \toprule
smashed(conserved edges)			&  166      &   1202     &    2356\\
smashed(time)								& 16.669   &    140.67   &    153.91\\
smashed(COGs predicted)				& 146         & 528       &   748\\
multi(conserved edges)					&2396     &   24254     &   30930\\
multi(time)										& 0.3972   &    18.306  &     24.434\\
multi(COGs predicted)                  	& 155      &   1045    &     1477\\ \bottomrule
\end{tabular}
\label{tab:5}
\caption{Human Mouse. 129862}
\end{table}




==> 99-Z-cut-text.tex <==
% Recently, we started seeing multimodal networks
Recently, we started observing a new dimension in networks, and that
is ``modality". 
A multimodal network (MMN) is a novel graph-theoretic formalism designed to
 capture the structure of biological networks and to represent relationships derived 
 from multiple biological databases~\cite{heath-multimodalnetworks}
 To understand modality, take the following example from biology, 
 annotating a relationship between two proteins can be based on 
protein sequence similarity, coocurrence in genes, coocurrence in scientific 
papers, experimental validation of interaction and more. 
Thus, each of these standards can be thought of as modes.
Multimodality appears in other scenarios; scientific papers repositories 
(papers are the nodes, references are the edges, and repositories are the modes), 
social media networks (users are the nodes, interactions are the edges, and social networks are the modes), 
transportation networks (stops are the nodes, direct routes are the edges, and methods of transportation are the modes) 
and many more.

The pairwise network alignment problem is formulated as follows: 
find a mapping between two networks satisfying the condition that no 
vertex in any of the networks receives more than one match, such that 
some similarity measure is maximized – in many cases,
 the topological similarity of the networks.
 The pairwise ``multimodal" network alignment problem adds an extra piece to the basic problem.
 Aside from satisfying the matching constraint and maximizing the similarity measure, 
 all nodes that are part of one mode from multimodal A can only map to nodes in one mode
  from multimodal B. 

There has been a number of pairwise network alignment algorithms that achieve very good results. From these, we mention~\cite{bayati-messagepassing} which uses belief propagation to solve the network alignment problem via maximizing the number of squares (or overlapped edges from both graphs). IsoRank[CCC] and NSD[CCC] (which is really a variant of IsoRank), are two other methods that use the idea of PageRank[CCC] 
to generate a similarity score on every pair of nodes from the two graphs. Theoretically, this is equivalent to running PageRank on the Kronecker graph of the two networks where each node in the PageRank solution vector corresponds to the similarity score between a pair of nodes from each of the input networks. [XXX should say these methods do not scale so well and thus we can't use them as they are on the multimodal networks]. As we will see later, multimodal networks tend to explode in size and thus existing pairwise network alignment algorithms cannot be readily used for the multimodal network alignment problem.

A multimodal network is a relatively new idea that encodes relationships between the same set of nodes that exist in multiple different databases. The hypothesis we validate in this paper is: If we have $k$ networks coming from $k$ databases, using multimodal alignment on these $k$ networks gives more indicative information rather than doing $k$ pairwise network alignment. 

%In~\cite{bayati-messagepassing}, 
%
%Both classes of methods, [CCC] and ([CCC],[CCC]), 
%
%require solving a matching problem after the solution to the system has been generated (the optimal value achieved in [CCC], and the PageRank solution in [CCC]). If the two networks in hand have $n$ nodes respectively, then storing the solution matrix $\mX$ requires $\mathcal{O}(n^2)$ storage. 

%This is one bottleneck 
%
%along with the repetitive matrix vector product in these iterative algorithms make using them on large scale datasets infeasible. 
%
%impose certain heuristics on the problem solve the network alignment problem to a 
%Many existing network alignment work very well for networks that are not of very large scale. By large scale, we mean a network of size $10^5$ or more. 
%Scalability is an issue that many traditional pairwise network alignment algorithms face. [XXX] uses belief propagation to solve
%the network alignment problem via maximizing  the number of squares (or overlapped edges). [XXX] shows the method used on 
%protein protein interaction networks and achieves high accuracy. However, the runtime of this alogrithm is $\mathcal{O}(n^3)$ where $n$
%is the size of the networks (for simplicity, assume that the two networks have the same size).
%IsoRank and NSD 
%(which is a variant of IsoRank) are two other methods used for network alignment . Both methods solve the network alignment problem by creating a similarity matrix $\mX$ and then solve a matching problem on $\mX$. If the two networks in hand have $n$ nodes respectively, then storing $\mX$ requires $\mathcal{O}(n^2)$ storage. This bottleneck along with the repetitive matrix vector product in these iterative algorithms make using them on large scale datasets infeasible. 
%
%A major bottleneck with the multimodal network alignment problem is the size of the networks. 
%These networks tend to be much bigger in size and thus traditional pairwise alignment algorithms cannot
%be readily used to perform multimodal network alignment.



Here, we describe how multimodal networks can be assembled from a set of input networks. 
Figure~\ref{figure:multimodalnetwork} illustrates the scenario when the number of modes is equal to 2.
In this example, assume that we have two networks (green and red on the left pannel).
Also, assume that we know that node $1$ in the green network is the same node number $1$ in the red network.
Similarly for the nodes $2$, $3$, and $4$. Looking at the left panel, we can see the adjacency matrices of each 
of these networks. To the right, we can see the multimodal network created. The block diagonal matrices in $\mM$ are the adjacency matrices of the previous networks. The elements on the off diagonal will have values $0$ or $1$ depending on the following. $\mM(i,j) = 1$ if $i$ and $j$ correspond to the same node in reality and $0$ otherwise. Since nodes $1$, $2$, $3$, and $4$ correspond to the same nodes in both networks we see $4$ $1's$ on the diagonal of the off diagonal block matrices of $\mM$.

\section{Notation}
XXX Add anything introduced later that needs to be put here.


%(Draw connections between the specific application to existing studies in the literature, clarify the constraints imposed by the application domain and distinguish your solutions from pre-existing ones in this context).
\section{Problem Setup}\label{problem-setup}
In this paper, we propose a multimodal network alignment method where the modal alignment is known apriori. We state the problem as follows. First, define two multimodal networks $\mM$ and $\mN$ where,
\begin{align*}
\mM = \bmat{\mM_1 & \mP_{1,2} & \hdots & \mP_{1,n} 
	\\ \mP_{1,2}^T & \mM_2 & \hdots & \mP_{2,n}
	\\ \vdots & \vdots & \vdots & \vdots
	\\ \mP_{1,n}^T & \mP_{2,n}^T & \hdots & \mM_n}
\end{align*}
\begin{align*}
\mN = \bmat{\mN_1 & \mQ_{1,2} & \hdots & \mQ_{1,n} 
	\\ \mQ_{1,2}^T & \mN_2 & \hdots & \mQ_{2,n}
	\\ \vdots & \vdots & \vdots & \vdots
	\\ \mQ_{1,n}^T & \mQ_{2,n}^T & \hdots & \mN_n},
\end{align*}
with $\mM_i$ and $\mN_i$ being the adjacency matrices of mode $i$ in $\mM$ and $\mN$ respectively, to be the input multimodal networks. The goal is to find an alignment between $\mM$ and $\mN$ that maximizes the topological similarity of the two networks.

We assume that we do not know anything about the similarity between the individual nodes but we know that nodes from mode $k$ in $\mM$ align to nodes from mode $k$ in $\mN$. We encode this property in a matrix $\mL$ that consists of $1's$ and $0's$ where the $(i,j)$ entry in $\mL$ is $1$ if node $i$ and node $j$ belong to the same mode and zero otherwise. $\mL$ can be written as follows,
\begin{align*}
\mL = \bmat{\mE  &\mZ & \hdots & \mZ 
	\\ \mZ & \mE & \hdots & \mZ
	\\ \vdots & \vdots & \vdots & \vdots
	\\ \mZ & \mZ & \hdots & \mE}
\end{align*}
where $\mE$ is the all ones matrix and $\mZ$ is the all zeros matrix. Note that $\mL$ has rank = $\# of modes$.\\



In the context described in section~\ref{sec:problem}, $\mL$ is a low-rank matrix of rank = $\# of modes = m$. Thus, $\mL$ can be represented as a sum of outer products. Specifically, 
\begin{align}
\mL = \bmat{\ve \\ 0 \\ 0 \\ \vdots \\ 0}  \cdot \bmat{\tilde{\ve} \\ 0 \\ 0 \\ \vdots \\ 0}^T + \hdots + \bmat{0 \\ 0 \\ \vdots \\ 0 \\ \ve}  \cdot \bmat{0 \\ 0 \\ \vdots \\ 0 \\ \tilde{\ve}}^T
\label{matrixL}
\end{align}
where $\ve$ and $\tilde{\ve}$ are the all ones vector. Note that $\ve$ and $\tilde{\ve}$ need not be of the same size.

We rewrite equation~\ref{eqn:NSD} to suit our multimodal setting:
\begin{equation}
\mX^{(t)} = (1-\alpha) \sum\limits_{k=0}^{t-1}\alpha^k \tilde{\mN}^k \mL (\tilde{\mM}^T)^k  + \alpha^t \tilde{\mN}^t \mL (\tilde{\mM}^T)^t
\end{equation}
where $\tilde{\mM}$ and $\tilde{\mN}$ are the normalized versions of $\mM$ and $\mN$. If the $i'th$ outer product from~\ref{matrixL} correspond to the vectors $\vw_i$ and $\vz_i$, and there are $t$ iterations, and the number of modes is $m$, then we can construct $\mU$ and $\mV$ such that:

\begin{equation}
\mU^T = 
\begin{bmatrix}
\vw_1 \\
(1-\alpha)\alpha \tilde{\mN} \vw_1 \\
\vdots \\
(1-\alpha)\alpha^{t-1} \tilde{\mN}^{t-1} \vw_1 \\
(1-\alpha)\alpha^{t} \tilde{\mN}^{t} \vw_1 \\
\vdots \\
\vw_n \\
(1-\alpha)\alpha \tilde{\mN} \vw_n \\
\vdots \\
(1-\alpha)\alpha^{t-1} \tilde{\mN}^{t-1} \vw_1 \\
(1-\alpha)\alpha^{t} \tilde{\mN}^{t} \vw_n
\end{bmatrix},
\mV^T = 
\begin{bmatrix}
\vw_1 \\
\tilde{\mM} \vw_1 \\
\vdots \\
\tilde{\mM}^{t-1} \vw_1 \\
\tilde{\mM}^{t} \vw_1 \\
\vdots \\
\vw_n \\
\tilde{\mM} \vw_n \\
\vdots \\
\tilde{\mM}^{t-1} \vw_1 \\
\tilde{\mM}^{t} \vw_n
\end{bmatrix},
\end{equation}

Hence, $\mX^{(t)} = \mU \mV^T$. Note that the construction of $\mU$ and $\mV$ uses multiple matrix vector products and no matrix matrix products. In the next section, we demonstrate how, when space is an issue, $\mU$ and $\mV$ can be utilized to compute a matching on the nodes of $\mM$ and $\mN$ withoug explicitly computing $\mX$.

%$\mV$ will be very similar to $\mU$, except that the vectors $\vz_i$ replace $\vw_i$ and the matrix $\mA$ replaces the matrix $\mB$. Assuming that $\mA$ and $\mB$ are the normalized matrices corresponding to the two input multimodal networks constructed as described in section~\ref{multi-creation}, $\mU$ and $\mV$ computed as above, then $\mU\mV^T$ is equivalent to the matrix $\mX$ as described in equation~\ref{eqn:IsoRank}. Also, note that the computation of $\mU$ and $\mV$ uses multiple matrix vector products and not matrix matrix products. We next describe how we use $\mU$ and $\mV$ to derive a matching on the networks.

%Algorithm 1 shows the pseudo code of the method. In this algorithm, we assume that $\mL = \sum\limits_{i = 1}^{i=n} \vw_i \vz_i^T$. $\mM$ and $\mN$ are the two input multimodal networks. The output of this algorithm will be $\mU$ and $\mV$ where the product $\mU\mV^T$ is equivalent to the matrix $\mX$ as described in equation~\ref{eqn:IsoRank}. Note that the implementation details differ. In specific, we do not perform any matrix matrix products.
%\begin{algorithm}
%  \caption{Multimodal Similarity Decomposition}
%%  \SetKwInOut{Input}{Input}
%\begin{algorithmic}[1]
%\Statex
%\INPUT
%\Statex $\mM$ %\Comment Multimodal 1
%\Statex $\mN$ 
%\Statex $\vw_i, \{i = 1,\hdots, n\}$
%\Statex $\vz_i, \{i = 1,\hdots, n\}$
%\Statex $\alpha$
%\Statex $maxiter$
%\State $\mV = 0$
%\State $\mU = 0$
%  \For {$i = 1 \textbf{ to } n$}
%  \For {$i = 1 \textbf{ to } maxiter$}
%  	\State $k = (maxiter+1)(i-1)+j$
%    	\State $\mU_{k} = (1-\alpha) \alpha^{j-1} \mB^{j-1} \vw_i$
%    	\State $\mV_{k} = \mA^{j-1} \vz_i$
%  \EndFor
%  \State $k = (maxiter+1)(i-1)+(maxiter+1)$
%  \State $\mU_{k} = \alpha^{maxiter} \mB^{maxiter} \vw_i$
%  \State $\mV_{k} = \mA^{j-1} \vz_i$
%  \EndFor
%  \end{algorithmic}
%\end{algorithm}
%As an example, if the system consists of 2 modes and the networks in each mode consist of 4 nodes, and the number of iterations is 1, then $\mU$ will be of size 8 - by - 4 and it will look like:
%\begin{align*}
%\mleft[
%\begin{array}{c|c|c|c}
%1 &  &0 & \\
%1 &  &0 & \\
%1 &  &0 & \\
%1 & c_1 \mB \vw_1 & 0 & c_1 \mB \vw_2\\
%0 &  &1 & \\
%0 &  &1 & \\
%0 &  &1 & \\
%0 &  &1 & \\
%\end{array}
%\mright]
%\end{align*}
%where $\vw_1 = \bmat{1\\1\\1\\1\\0\\0\\0\\0}$, $\vw_2 = \bmat{0\\0\\0\\0\\1\\1\\1\\1}$, and $c_1 = (1-\alpha)\alpha$



\subsection{Resolving matching conflicts}
Once we have $\mU$ and $\mV$ from the multimodal similarity decomposition, we will produce a matching from them as described 

\label{sec:conflict} 
We compute a multimodal similarity decomposition as a low-rank solution of the IsoRank matrix $\mY$ computed with respect to the multimodal adjacency matrices $\mM$

Singh et al. in~\cite{singh2008-isorank-multi} propose IsoRank which builds on PageRank[CCC] to derive similarity scores between pairs of nodes from two networks. IsoRank relies on an iterative procedure of the form: 
\begin{align}
\mX = \alpha \mB \mX \mA^T + (1-\alpha) \mL
\label{eqn:IsoRank}
\end{align}
$\mA$ and $\mB$ are the column stochastic normalized adjacency matrices of the two networks. $\mL$ is a prior known measure of similarity between the pairs of nodes from $\mA$ and $\mB$. $(1 - \alpha)$ represents a confidence measure in the matrix $\mL$, it is analogous to the teleportation parameter in the PageRank equation. $\mX(i,j)$ at a certain iteration is the similarity measure between node $i$ in the network corresponding to $\mB$ and node $j$ in the network corresponding to $\mA$. Setting $\mX^{(0)}=\mL$ and expanding the iterations of equation~\eqref{eqn:IsoRank} yields:
\begin{equation}
\mX^{(t)} = (1-\alpha) \sum\limits_{k=0}^{t-1}\alpha^k \mB^k \mL (\mA^T)^k  + \alpha^t \mB^t \mL (\mA^T)^t
\label{eqn:IsoRank_expanded}
\end{equation}
Network Similarity Decomposition (NSD) introduced in~\cite{Kollias-2011-netalign} shows a similarity decomposition strategy to decompose the similarity matrix $\mL$ and thus improve the runtime of the algorithm.~\cite{Kollias-2011-netalign} write $\mL$ as a summation of rank-1 matrices. Specifically, if $\mL = \sum\limits_{i=1}^{i=s}\vw_i\vz_i^T$, equation~\ref{eqn:IsoRank_expanded} can be rewritten as
\begin{equation}
\mX^{(t)} = (1-\alpha) \sum\limits_{k=0}^{t-1}\alpha^k \vw_i^{(k)} \vz_i^{{(k)}^T}  + \alpha^t\vw_i^{(t)} \vz_i^{{(t)}^T}
\label{eqn:NSD}
\end{equation}
where $\vw_i^{(k)} = \mB^k\vu_i$ and $\vz_i^{(k)} = \mA^k\vz_i$.\\

NSD improves on IsoRank by performing this low-rank decomposition but it still faces one bottleneck after the computation of the similarity matrix $\mX$. This bottleneck is to solve a matching problem on the solution ($\mX$) of this system. Multiple methods can be used to solve the matching problem on $\mX$, nevertheless, since $\mX$ is a dense matrix, it might be infeasible to store $\mX$ and solve for a matching on it for large-scale networks.



%In this paper, we propose an new matching approximation that doesn't require storing all entries of the matrix $\mX$, but instead, uses the low-rank representation of $\mX = \mU\mV^T$. Then we use this method to perform multimodal network alignment and validate the hypothesis that the multimodal network alignment solution can be stronger than the multiple uni-modal network alignment solutions combined. In this paper, we build on the NSD algorithm but we drop the step of constructing the matrix $\mX$.
The multimodal network alignment problem as presented in Section~\ref{sec:problem} assumes aprior knowledge of the modal alignment but no apriori knowledge of the relationship between the nodes. Here, we translate the problem to the following: Given two multimodal networks $\mM$ and $\mN$ of the form shown in equation~\ref{eqn:multimodalmatrix}, and a similarity matrix $\mL$ of the form shown in equation~\ref{eqn:matrixL}, where $\mE$ is the all ones matrix and $\mZ$ is the all zeros matrix, produce an alignment that maximizes the overlap of the two networks. Note that without loss of generality, $\mL$ implicitly assumes that mode $i$ in $\mM$ aligns to node $i$ in $\mN$.
\begin{equation}
\mL = \bmat{\mE  &\mZ & \hdots & \mZ 
	\\ \mZ & \mE & \hdots & \mZ
	\\ \vdots & \vdots & \vdots & \vdots
	\\ \mZ & \mZ & \hdots & \mE}
\label{eqn:matrixL}
\end{equation}



This means that we easily compute a $1/k$-approximate matching by 

The bipartite matching problem on two networks $\mA$ and $\mB$ can be stated as follows: Given a similarity score between every pair of nodes from $\mA$ and $\mB$, find a matching on the two networks that maximizes the total weight. The score information can be encoded in a matrix (call it $\mX$), and the the value $\mX(i,j)$ represents the similarity score between node $i$ in network $\mA$ and node $j$ in network $\mB$. Computing the maximum weighted matching on $\mX$ is a problem that has been widely studied in the past and a number of exact polynomial time algorithms have been developed. Eventhough polynomial time algorithms exist for this problem, using them might be infeasible in cases when the networks are too large[CCC Maue and Sanders]. This reason motivated the use of approximation algorithms for the maximum weighted matching problem (which normally requires a lower runtime and achieves very good results empirically).

In the context of multimodal network alignment, whether an exact or approximate algorithm is chosen to perform the matching, there will be a bottleneck before the algorithm even starts. And this bottlenech is the construction of the matrix $\mX$. In the context of our pipeline, $\mX = \mU\mV^T$. Note that if $\mU$ and $\mV$ are of size $n by k$ each, then there are $\mathcal{O}(n^2k)$ operations to construct the matrix. Moreover, storing this matrix will require $\mathcal{O}(n^2)$ space whereas storing $\mU$ and $\mV$ requires $\mathcal{O}(nk)$.

In this section, we describe three approaches to solve the matching problem on a matrix, where the low rank representation of the matrix is given instead of the matrix itself. (i.e. given $\mU$ and $\mV$ such that $\mU\mV^T = \mX$, find an approximate matching on $\mX$ without computing $\mX$). The methods that follow in this section make use of the following theorem.
\begin{theorem} Let $f$ be the maximum weighted matching function on a matrix $\mA$. Then $f(|\mA|)$ is a matrix norm.\label{thm:mwm-norm}\end{theorem}
\begin{proof} Note that $|\mA|$ is a nonzero matrix.
	\begin{enumerate}[i]
		\item $f(|\mA|) = \max\limits_{M} ( \sum\limits_{i,j}{|a_{ij}|})$, where $M$ is the set of all possible matchings. Since $|a_{ij}|$ are always non-negative, their summation is always non-negative, and thus $f(|\mA|)\geq0$.
		\item If $|\mA| = 0$, then $\max\limits_{M} ( \sum\limits_{i,j}0) = 0$, and thus $f(|\mA|)=0$.\\
		If $\max\limits_{M} ( \sum\limits_{i,j}{|a_{ij}|}) = 0$, then $a_{ij} = 0  \forall i,j$. Thus, $\mA = 0$.
		\item $f(|c\mA|) = \max\limits_{M} ( \sum\limits_{i,j}{|ca_{ij}|}) = |c| \max\limits_{M} ( \sum\limits_{i,j}{|a_{ij}|}) = |c|f(|\mA|)$
		\item (Proof of $f(|\mA + \mB|) \leq f(|\mA|) + f(|\mB|)$). Let $\mC = \mA + \mB$. Then there exists a permutation matrix $\mP_C$ such that $f(|\mC|) = \sum_{i}\sum_{j} \mP_C \circ |\mC|$ where $\circ$ represents the Hadamard product of the two matrices. Similarly, there exists two permutation matrices $\mP_A$ and $\mP_B$, where $f(|\mA|) = \sum_{i}\sum_{j} \mP_A \circ |\mA|$ and $f(|\mB|) = \sum_{i}\sum_{j} \mP_B \circ |\mB|$.\\
		Since $\mP_A$ attains the maximum weighted matching for the matrix $\mA$, then\\
		$\sum_{i}\sum_{j} \mP_C \circ |\mA| \leq \sum_{i}\sum_{j} \mP_A \circ |\mA|$.\\
		Similarly for the matrix $\mB$,\\
		$\sum_{i}\sum_{j} \mP_C \circ |\mB| \leq \sum_{i}\sum_{j} \mP_B \circ |\mB|$.\\
		Combining the above equation and substituting $(\mA+\mB)$ instead of $\mC$ leads to:\\
		$\sum_{i}\sum_{j} \mP_C \circ |\mC| = \sum_{i}\sum_{j} \mP_C \circ |\mA + \mB|$\\
		$ \leq\sum_{i}\sum_{j} \mP_C \circ |\mA| +\sum_{i}\sum_{j} \mP_C \circ |\mB|$.\\
		$\leq \sum_{i}\sum_{j}  \mP_A \circ |\mA| + \sum_{i}\sum_{j} \mP_B \circ |\mB|$\\
		$ = f(|\mA|) + f(|\mB|)$
	\end{enumerate}
\end{proof}

\begin{prop}
	Let $\mK = \vu \vv^T$ be a rank-1 matrix, then the maximum weighted matching on $\mK$ can be achieved by sorting $\vu$ and $\vv$ and computing the dot product of the sorted vectors (if $\vu$ and $\vv$ are of the same size). If the vectors are of different sizes, and the smaller size is $l$, then the maximum weighted matching is the dot product of the top $l$ elements.
	\label{prop:rearrangement}
\end{prop}
\begin{proof}
	This follows immediately from the rearrangement inequality. [CCC]
	%Hardy, G.H.; Littlewood, J.E.; Pólya, G. (1952), Inequalities, Cambridge Mathematical Library (2. ed.), Cambridge: Cambridge University Press, ISBN 0-521-05206-8, MR 0046395, Zbl 0047.05302, Section 10.2, Theorem 368
\end{proof}


\subsection{Matching Approximations}
This approximation follows from theorem~\ref{thm:mwm-norm} and makes use of proposition~\ref{prop:rearrangement}. Recall that $\mX = \mU \mV^T =  \sum\limits_{i=1}^k \vu_i\vv_i^T$. Let $f$ be the maximum weighted matching function defined on the matrix $\mX$. Using theorem 7.1, we can state the following
\begin{align}
f(\mX) \leq f(\mX_1) + f(\mX_2) + \hdots + f(\mX_k)
\end{align}
where $\mX_k = \vu_k \vv_k^T$.\\
There exists an index $s$, $1\leq s \leq  k$, such that $f(\mX_s) \geq f(\mX_i) \forall i \in \{1 \hdots k \}$, then
\begin{align}
f(\mX) \leq f(\mX_1) + f(\mX_2) + \hdots + f(\mX_k) \\
\leq f(\mX_s) + \hdots + f(\mX_s) = k f(\mX_s)
\end{align}
Thus, $f(\mX_s) \geq 1/k f(\mX_s)$, and hence the best maximum weighted matching from the $k$ outer products achieves a $1/k$ approximation of the matching on $\mX$.
\begin{algorithm}
	\caption{(1/k) - approximation}
	\begin{algorithmic}
		\For {$i = 1 : k$}
		\State $\tilde{\vu}_i$ = sort $(\vu_i)$
		\State $\tilde{\vv}_i$ = sort $(\vv_i)$
		\State $c = \min (length((\vu_i), length((\vv_i))$
		\State $\vw(i) = \sum\limits_{j = 1}^{j = c} \tilde{\vu}_i(j) \tilde{\vv}_i(j)$
		\EndFor
		\State $s = \text{argmax}(\vw)$
	\end{algorithmic}
	\label{alg:1k-approximation}
\end{algorithm}

Algorithm~\ref{alg:1k-approximation} shows a simple pseudo code to obtain the index of the outer product that achieves a $1/k$ maximum weighted matching approximation. In Algorithm~\ref{alg:1k-approximation}, $\vu_i$ and $\vv_i$ are the $i'th$ columns of $\mU$ and $\mV$ respectively. If $\mU$ and $\mV$ are each size $n by k$ each, then, the runtime complexity of Algorithm~\ref{alg:1k-approximation} is $\mathcal{O} (kn \log{} n)$, and the space requirement is $\mathcal{O} (kn)$. The output of Algorithm~\ref{alg:1k-approximation} is the index of matching that achieves the the $1/k$ approximation. Although this approximation has a guaranteed theoretical bound on the weight, it is useful to use the generated $k$ pairs of vectors to produce better matchings at a low cost. For the rest of this section, we assume that $\mU$ and $\mV$ are of size $n by k$ each for similicity of notation.

\paragraph{Global Maximum Weight}
Algorithm~\ref{alg:1k-approximation} produces $k$ valid matchings. This variant evaluates all the generated $k$ matchings on $\mU$ and $\mV$ and keeps the one with the highest weight. To see that this retains the $1/k$ bound, assume that the best matching from the $s'th$ outer product applied on the $s'th$ outer product achieves a weight of $W_s$, then if we apply it on the rest of the outer products, we achieve a new weight $W_s + \Delta$. Since $W_s + \Delta > W_s$, and $W_s \geq 1/k W^*$ where $W^*$ is the maximum weight possible, then $W_s + \Delta > 1/k W^*$. If there is another matching (call it the $t'th$ matching) from the $k$ matchings that achieves a higher weight than $W_s + \Delta$, then the $t'th$ matching achieves a total weight higher than $1/k W^*$.

\textbf{Runtime.} To evaluate one matching, this requires $\mathcal{O}(nk)$ operations. To evaluate $k$ of them, this requires $\mathcal{O}(nk^2)$. Adding the runtime of Algorithm~\ref{alg:1k-approximation}, this yields $\mathcal{O}(nk^2 + kn \log{} n)$

\paragraph{Matchings Union}
The key idea of this variant is to take the union of the previously generated $k$ matchings. Each matching generates $n$ node matches, so, in total, the $k$ matchings generate $nk$ possible pairs. This method picks the top $n$ matches out of these $nk$ possible pairs by sequentially picking the highest weighted edges first while insuring that the matching constraint is not compromised.

\textbf{Runtime.} To evaluate one of the weights of the $nk$ edges, this requires $\mathcal{O}(k)$ operations. Since there are $nk$ edges, then the total runtime is $\mathcal{O}(nk^2)$. Since we need to sort these edges afterwards, there is an additional $\mathcal{O}(kn\log{} kn)$ requirement and thus the total runtime would be $\mathcal{O} (nk^2 + kn\log{} kn)$. Adding the runtime of Algorithm~\ref{alg:1k-approximation} doesn't change the current bound.


\paragraph{Global overlap of matchings}
The base Algorithm (Algorithm~\ref{alg:1k-approximation}) and the two variants (global maximum weight and matchings union) approach the problem trying to maximize the total weight of the matching. In problems like network alignment, one might be interested in the total size of the overlap between the two networks after the matching has been applied on both networks. For that reason we consider a new metric to evaluate each of the matchings, which is the size of the overlapped edges. More concretely, we apply the matching pairs independently and count the size of the edge overlap. The matching with the highest value of edge overlap becomes the winner.

\textbf{Runtime.} To evalute one matching on the networks, this requires $\mathcal{O} (nnz_1 + nnz_2)$, where  $nnz_1$ and $nnz_2$ represent the number of nonzeros in the networks. To evaluate $k$ matchings, this requires $\mathcal{O} (kn\log{} n + k (nnz_1 + nnz_2))$. Adding the contribution from Algorithm~\ref{alg:1k-approximation} 1, this leads to a total runtime of $\mathcal{O} (kn\log{} n + k (nnz_1 + nnz_2))$


\subsection{Data Description}
We explore an airline transportation network obtained from two sources. In specific, we obtain the first dataset from; we use the continental mutiplex airline transportation network of Europe. In this dataset, there are 175 layers modes, where each mode corresponds to an airline. The total number of airports present in this multiplex network is 594. In this dataset, the airports have been anonymized whereas the airlines information is still known. The second dataset comes from the Openflights repository [CCC] and we use the version from May 2013 (~\cite{Nicosia-2015-multiplex} was first published in 2014, so we looked for datasets that were closer to that date). In ~\cite{Nicosia-2015-multiplex}, the data was acquired from the Openflights dataset and thus an exact alignment between these two datasets should exist. Next, we filtered the airports dataset obtained from [CCC] to contain airports that are located in Europe. We then used these airports to filter the routes dataset based on the condition that the start and end point of a certain route must be an airport that is located in Europe. Unlike the dataset from~\cite{Nicosia-2015-multiplex}, here, we know the actual identity of the airports as well as the airlines. The end goal of this experiment was to be able to de-anonymize the data in the first dataset. Before we proceed with the alignment of these networks, we make the two networks undirected, i.e. for every directed edge, we add an edge in the opposite direction.
\subsection{Global Alignment}
To perform global alignment on these two networks, we create two multimodal networks as described in Section~\ref{sec:problem}. We then normalize the networks and compute $\mU$ and $\mV$ as described in Section~\ref{sec:msd}. Then, since these networks were very large, we use the methods from ~\ref{sec:matching} applied on $\mU$ and $\mV$ to compute a matching on the networks. 

%Using this dataset only, we know which networks correspond to which airlines; on the other hand, the airports have been anonymized with arbitrary indices. The second dataset comes from the Openflights repository [CCC], [CCC](Nicosia) mentions that the data obtained in their dataset is from the openflight repository and thus, obtaining the data from the source of openflights should give the same networks. Since [CCC](Nicosia) was published in 2014, we looked for the earlier commits of the data. We found that the commit from May 2013 was the only one that included all the layers included in [CCC] Nicosia's dataset and hence we chose that dataset to proceed with. 
%The first dataset was obtained from [XXX] \textit{http://www.maths.qmul.ac.uk/~vnicosia/sw.html} and Openflights repository \textit{https://github.com/jpatokal/openflights} [XXX talk more about the data]. Task was to deanonymize the datasets.

10,25,50,100
\begin{table}[h]
	\centering
	\begin{tabular}{rllll}
		\toprule
		\textbf{Method}                        & \textbf{\#edges} & \textbf{weight}\\ \toprule
		Max Weight                 & $6468$ & $1.3328$\\
		Matching Union           & $6468$ & $1.3328$\\
		Max Overlap               & $6468$ & $1.3328$\\ \bottomrule  \\
	\end{tabular}
	\label{tab:1}
	\caption{This table shows the size of the overlap achieved after applying the matchings on the two networks. All matchings perform the same. The total size of overlap of these networks is 6468, and thus all method achieve the best alignment. All of these methods run in under a minute on [XXX computer specs?]. The total weight achieved by the three methods is the same[XXX fix this sentence/define weight]. The number of iterations that was used in these experiments is 5 iterations and $\alpha = 0.2$. For the rest of this section, we use our multimodal alignment method with the matching union approach[XXX fix this sentence and move it outside of caption]}
\end{table}
%\textbf{A comment on the bipartite matching result.} Since the two network are exactly the same we were expecting that all algorithms get all the edges, but bipartite matching didn't get all the data so we investigated this discripancy. Having missed 12 edges essentially means that 6 undirected edges were missed since the network is symmetric. Looking for these 6 edges, we found that they were missed in 3 modes (i.e. in 3 modes, 2 edges were swapped). These three modes were of sizes 1476, 20 and 208. [XXX, explaing this better? The structure that messed things up was a triangle]
\begin{figure}[h]
	\centering
	\includegraphics[scale=0.4]{smash}
	\caption{Illustration of smashing a multimodal network}
	\label{figure:smash}
\end{figure}

\subsubsection{Comparison with state-of-the-art methods}
To assess the effectiveness of the multimodal alignment method we presented, we compared our results with existing methods for network alignment. 

Next, we wanted to assess the effectiveness of multimodality, so we devised  a new experiment. In the context of the Airlines dataset, which contains 175 networks, a natural solution could be to assemble all the networks in one network. We refer to this approach as the smashed version of the networks. Figure~\ref{fig:smash} illustrates the idea. In the airlines networks scenario, we smash both multimodal networks and then use an existing network alignment method to align these networks. We ran IsoRank and netalignmr[XXX citation here] on the smashed networks. Another natural solution to solve the multimodal network alignment problem when the modal alignment is known is to perform pairwise alignment on each pair of the modes. We refer to this method as the multi pairwise alignment. We evaluate this method by successively aligning the networks $\mA_s$ and $\mB_s$ and applying the matching obtained on all the other pairs. We then pick the matching that achieved the highest overlap value. We run the multi pairwise alignment method with IsoRank and netalignmr as well. We report all the scores in table


In Figure~\ref{figure:smashresult}, we see the number of conserved edges of the pairwise network alignment as the number of iterations of netalignmr increase. The total number of possible edges to recover is 8340 (note that this number is different from the total number of edges in the multimodal case is due to smashing the networks and thus some edges overlapped). We can see that the multimodal alignment result was superior.

\subsubsection{Multimoal Alignment versus multiple uni-modal alignment}
To investigate the strength of multimodal alignment even further we wanted to look at the pairwise network alignment result of each of the 175 networks. We used the 3 matching variants, bipartite matching and netalignmr to conduct this experiment. In many of the networks, the five methods have indeed recovered all the possible edges in the network, but failed on a number of them. In table~\ref{tab:2} we show the number of conserved edges of the best matching variant, bipartite matching and netalignmr for some of the modes. From simply looking at this table we can see that the aggregation of the missed edges from bipartite matching for example is more than 12 edges (or 6 undirected). We next wanted to verify what happens as more and more modes enter the alignment process. We ran 100 random experiments that solved the multimodal alignment problem as the number of modes increased. We report the results in Figure~\ref{figure:smash}.


\begin{table}[h]
	\centering
	\begin{tabular}{rllll}
		\toprule
		\textbf{mode}                        & \textbf{1/k} & \textbf{BM} & \textbf{smashed} & \textbf{total}\\ \toprule
		3                             & 34 & 38 & 32 & 38\\
		12                 & 28 & 28 & 28 & 32\\
		17                  & 480 & 468 & 398 & 480\\
		32                  & 4 & 4 & 4 & 8\\
		41                  & 142 & 146 & 146 & 146\\
		42                  & 8 & 12 & 16 & 16\\
		43                  & 4 & 4 & 4 & 8\\
		82                  & 592 & 524 & 502 & 596\\
		108                  & 0 & 0 & 0 & 6\\
		127                     & 2 & 2 & 4 & 6\\ \bottomrule
	\end{tabular}
	\label{tab:2}
	\caption{This table shows the results of network alignment performed on a selection of modes.}
\end{table}

\begin{figure}
	\centering
	\includegraphics[scale=0.45]{ROG.eps}
	\caption{ROG plot of 100 experiments XXX fix caption}
	\label{figure:ROG}
\end{figure}

%Looking at this table at a first glance, we can see that that multimodal alignment actually helped because pairwise alignment missed more than one edges... bla bla. We look more closely at this phenomenon via the next experiment. The point of the next experiment is: the more modes the better the alignmetn is.
%
%What we do here is that we take a bunch of 5 modes that don't achieve full ...
%
%We can notice from this table that aligning


==> hudaDef.tex <==
%new commands defined by Huda
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{cancel}

\usepackage{listings}
\usepackage{color} %red, green, blue, yellow, cyan, magenta, black, white
\definecolor{mygreen}{RGB}{28,172,0} % color values Red, Green, Blue
\definecolor{mylilas}{RGB}{170,55,241}
\renewcommand{\qedsymbol}{\rule{1ex}{1ex}}

\newcommand{\putInBox}[1]{

\noindent\fbox{%
    \parbox{\textwidth}{%
        {#1}
    }%
}
}

\lstset{language=Matlab,%
    basicstyle=\footnotesize\ttfamily,
    breaklines=true,%
    morekeywords={matlab2tikz},
    keywordstyle=\color{blue},%
    morekeywords=[2]{1}, keywordstyle=[2]{\color{black}},
    identifierstyle=\color{black},%
    stringstyle=\color{mylilas},
    commentstyle=\color{mygreen},%
    showstringspaces=fa\\
    e,%without this there will be a symbol in the places where there is a space
    numbers=left,%
    numberstyle={\tiny \color{black}},% size of the numbers
    numbersep=9pt, % this defines how far the numbers are from the text
    emph=[1]{for,end,break},emphstyle=[1]\color{red}, %some words to emphasise
    %emph=[2]{word1,word2}, emphstyle=[2]{style},    
}



%finish commands defined by Huda

==> preamble-sdm.tex <==
\usepackage{ltexpprt}
\usepackage{mleftright}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% packages added by Huda - START
\usepackage{graphicx}
\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{enumerate}
\usepackage{booktabs}

\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\INPUT{\item[\algorithmicinput]}

\newtheorem{prop}{Proposition}

% packages added by Huda - END
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> preamble1.tex <==
%\usepackage{geometry}
%\geometry{letterpaper,textwidth=350pt,textheight=680pt,tmargin=60pt,
%            left=72pt,right= 72pt, footskip=24pt,headsep=18pt,headheight=14pt}
%            
%            
%            \usepackage[letterpaper,margin=1.5in,tmargin=1in,bmargin=1in]{geometry}
%or
%\geometry{letterpaper,margin=1.75in,tmargin=1in,bmargin=1in}
%\usepackage[letterpaper,margin=1.75in,tmargin=1in,bmargin=1in]{geometry}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{textcase}
\usepackage{soul}

%% THINGS KYLE HAS ADDED
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\inv}{^{-1}}
\newcommand{\mynt}{ {\color{red} Note:} }
\newcommand{\myans}{{\color{blue}\textbf{Answer}}\newline}
\DeclareMathOperator{\rank}{rank}

%%


\newcommand{\mat}[1]{\boldsymbol{#1}}
\renewcommand{\vec}[1]{\boldsymbol{\mathrm{#1}}}
\newcommand{\vecalt}[1]{\boldsymbol{#1}}

\newcommand{\conj}[1]{\overline{#1}}

\newcommand{\normof}[1]{\|#1\|}
\newcommand{\onormof}[2]{\|#1\|_{#2}}

\newcommand{\itr}[2]{#1^{(#2)}}
\newcommand{\itn}[1]{^{(#1)}}

\newcommand{\eps}{\varepsilon}
\newcommand{\kron}{\otimes}

\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\tvec}{vec}

\newcommand{\prob}{\mathbb{P}}
\newcommand{\probof}[1]{\prob\left\{ #1 \right\}}

\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\spmat}[1]{\left(\begin{smallmatrix} #1 \end{smallmatrix}\right)}
\newcommand{\sbmat}[1]{\left[\begin{smallmatrix} #1 \end{smallmatrix}\right]}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}

\renewcommand{\baselinestretch}{1} 

\providecommand{\eye}{\mat{I}}
\providecommand{\mA}{\ensuremath{\mat{A}}}
\providecommand{\mB}{\ensuremath{\mat{B}}}
\providecommand{\mC}{\ensuremath{\mat{C}}}
\providecommand{\mD}{\ensuremath{\mat{D}}}
\providecommand{\mE}{\ensuremath{\mat{E}}}
\providecommand{\mF}{\ensuremath{\mat{F}}}
\providecommand{\mG}{\ensuremath{\mat{G}}}
\providecommand{\mH}{\ensuremath{\mat{H}}}
\providecommand{\mI}{\ensuremath{\mat{I}}}
\providecommand{\mJ}{\ensuremath{\mat{J}}}
\providecommand{\mK}{\ensuremath{\mat{K}}}
\providecommand{\mL}{\ensuremath{\mat{L}}}
\providecommand{\mM}{\ensuremath{\mat{M}}}
\providecommand{\mN}{\ensuremath{\mat{N}}}
\providecommand{\mO}{\ensuremath{\mat{O}}}
\providecommand{\mP}{\ensuremath{\mat{P}}}
\providecommand{\mQ}{\ensuremath{\mat{Q}}}
\providecommand{\mR}{\ensuremath{\mat{R}}}
\providecommand{\mS}{\ensuremath{\mat{S}}}
\providecommand{\mT}{\ensuremath{\mat{T}}}
\providecommand{\mU}{\ensuremath{\mat{U}}}
\providecommand{\mV}{\ensuremath{\mat{V}}}
\providecommand{\mW}{\ensuremath{\mat{W}}}
\providecommand{\mX}{\ensuremath{\mat{X}}}
\providecommand{\mY}{\ensuremath{\mat{Y}}}
\providecommand{\mZ}{\ensuremath{\mat{Z}}}
\providecommand{\mLambda}{\ensuremath{\mat{\Lambda}}}
\providecommand{\mPbar}{\bar{\mP}}

\providecommand{\ones}{\vec{e}}
\providecommand{\va}{\ensuremath{\vec{a}}}
\providecommand{\vb}{\ensuremath{\vec{b}}}
\providecommand{\vc}{\ensuremath{\vec{c}}}
\providecommand{\vd}{\ensuremath{\vec{d}}}
\providecommand{\ve}{\ensuremath{\vec{e}}}
\providecommand{\vf}{\ensuremath{\vec{f}}}
\providecommand{\vg}{\ensuremath{\vec{g}}}
\providecommand{\vh}{\ensuremath{\vec{h}}}
\providecommand{\vi}{\ensuremath{\vec{i}}}
\providecommand{\vj}{\ensuremath{\vec{j}}}
\providecommand{\vk}{\ensuremath{\vec{k}}}
\providecommand{\vl}{\ensuremath{\vec{l}}}
\providecommand{\vm}{\ensuremath{\vec{l}}}
\providecommand{\vn}{\ensuremath{\vec{n}}}
\providecommand{\vo}{\ensuremath{\vec{o}}}
\providecommand{\vp}{\ensuremath{\vec{p}}}
\providecommand{\vq}{\ensuremath{\vec{q}}}
\providecommand{\vr}{\ensuremath{\vec{r}}}
\providecommand{\vs}{\ensuremath{\vec{s}}}
\providecommand{\vt}{\ensuremath{\vec{t}}}
\providecommand{\vu}{\ensuremath{\vec{u}}}
\providecommand{\vv}{\ensuremath{\vec{v}}}
\providecommand{\vw}{\ensuremath{\vec{w}}}
\providecommand{\vx}{\ensuremath{\vec{x}}}
\providecommand{\vy}{\ensuremath{\vec{y}}}
\providecommand{\vz}{\ensuremath{\vec{z}}}
\providecommand{\vpi}{\ensuremath{\vecalt{\pi}}}

\sodef\allcapsspacing{\upshape}{0.15em}{0.65em}{0.6em}%

%\makeatletter
%\def\maketitle{%
%\par
%\hrule height 0.75pt\vspace{1ex}
%\par\noindent
%%\begin{minipage}{0.5\textwidth}
%%\scshape
%%\textit{\@author}\\[0.2ex]\\
%%\textit{\@date}\\
%%CS 52500 HW1\\
%%\end{minipage}
%\begin{minipage}{1\textwidth}
%\raggedleft
%\textit{\@author}\\[0.2ex]
%\textit{\@title}\\
%\textit{\@date}
%\end{minipage}
%\par\vspace{1ex}
%\hrule height 1pt
%\vspace{2ex}
%\par
%}
%\input{hudaDef.tex}
%\makeatother
%
%\author{Huda Nassar \href{mailto:hnassar@purdue.edu}{hnassar@purdue.edu}}
%\title{SIAM Data Mining Draft - Multimodal Network Alignment}
%% auto generate a title
%\AtBeginDocument{\maketitle}
